Non-Intrusive Reduced-Order Modeling Using Uncertainty-Aware Deep Neural Networks and Proper Orthogonal Decomposition: Application to Flood Modeling

Deep Learning research is advancing at a fantastic rate, and there is much to gain from transferring this knowledge to older fields like Computational Fluid Dynamics in practical engineering contexts. This work compares state-of-the-art methods that address uncertainty quantification in Deep Neural Networks, pushing forward the reduced-order modeling approach of Proper Orthogonal Decomposition-Neural Networks (POD-NN) with Deep Ensembles and Variational Inference-based Bayesian Neural Networks on two-dimensional problems in space. These are first tested on benchmark problems, and then applied to a real-life application: flooding predictions in the Mille \^Iles river in the Montreal, Quebec, Canada metropolitan area. Our setup involves a set of input parameters, with a potentially noisy distribution, and accumulates the simulation data resulting from these parameters. The goal is to build a non-intrusive surrogate model that is able to know when it does not know, which is still an open research area in Neural Networks (and in AI in general). With the help of this model, probabilistic flooding maps are generated, aware of the model uncertainty. These insights on the unknown are also utilized for an uncertainty propagation task, allowing for flooded area predictions that are broader and safer than those made with a regular uncertainty-uninformed surrogate model. Our study of the time-dependent and highly nonlinear case of a dam break is also presented. Both the ensembles and the Bayesian approach lead to reliable results for multiple smooth physical solutions, providing the correct warning when going out-of-distribution. However, the former, referred to as POD-EnsNN, proved much easier to implement and showed greater flexibility than the latter in the case of discontinuities, where standard algorithms may oscillate or fail to converge.

==> content/podbnn-results.tex <==
\subsection{Setup and results}
\begin{figure}[t]
  \fbox{
    \parbox{\textwidth}{
\includegraphics[width=\linewidth]{images/podbnn-ackley-graph-meansamples.pdf}
    }
  }
  \\ \parbox{\textwidth}{
\caption{Identical setup as Figure \ref{fig:podensnn-ackley-graph-samples}, second column samples in the scope and third column out-of-distribution, yet with Bayesian Neural Network regression} 
    \label{fig:podbnn-ackley-graph-samples}
  }
\end{figure}
% \begin{figure}[t]
%   \centering
%   \fbox{
%   %  \includegraphics[width=0.45\textwidth]{images/podensnn-sw-far-1.png}
%   %  \hspace{0.04\textwidth}
%   %  \includegraphics[width=0.45\textwidth]{images/podensnn-sw-close-1.png}
%    \parbox{\linewidth}{
%     \subfloat[Random test sample on two different locations, incoming flow of $Q=1159.8$]{
%      \includegraphics[width=0.468\linewidth]{images/podensnn_map_zoom_a_1}
%      \hspace{0.04\linewidth}
%      \includegraphics[width=0.468\linewidth]{images/podensnn_map_zoom_b_1}
%     }
%     }
%   }
% \\ \parbox{1.\textwidth}{
%     \caption{POD-BNN of the same flood modeling application. The red line symbolizing the true simulated value, and the light blue representing 2 added standard deviations} \label{fig:podbnn-sw-map-1}
% }
% \end{figure}
\begin{figure}[t]
  \centering
  \resizebox{0.95\textwidth}{!}{
  \fbox{
    \parbox{\textwidth}{
    \parbox{\linewidth}{
    \subfloat[View from afar of a random test sample $Q=884.4\ \textrm{m}^3/\textrm{s}$. This shows an iso-contour at $h=0.05\ m$, with its boundary being the flooding lines. For illustration purposes, the overall predicted relative water height $h_\textrm{pred}$ has been pictured throughout. The green boxes show the two different locations of the following closer shots]{
   \includegraphics[width=\linewidth]{images/podensnn_map_wide}
    }
  }
  % \vspace{5mm}
    \parbox{\linewidth}{
  \subfloat[Random test sample with two levels of zoom, incoming flow of $Q=884.4\ \textrm{m}^3/\textrm{s}$]{
   \includegraphics[width=0.468\linewidth]{images/podbnn_map_zoom_a_1}
   \hspace{0.04\linewidth}
   \includegraphics[width=0.468\linewidth]{images/podbnn_map_zoom_b_1}
    }
  }
  % \vspace{-5mm}
    \parbox{\linewidth}{
  \subfloat[Random test sample with two levels of zoom, incoming flow of $Q=1159.8\ \textrm{m}^3/\textrm{s}$]{
   \includegraphics[width=0.468\linewidth]{images/podbnn_map_zoom_a_2}
   \hspace{0.04\linewidth}
   \includegraphics[width=0.468\linewidth]{images/podbnn_map_zoom_b_2}
    }
  }
  }
    }
  }
\\ \parbox{\textwidth}{
    \caption{POD-BNN application: flood modeling on the Mille Îles river. Flooding lines at $h=0.05\ m$ are shown on the close-up shots, with the red one for the CuteFlow solution, and the white ones representing the end of the predicted confidence interval $\pm2\sigma_D$. The distance between the simulated value and the upper bound is measured} \label{fig:podbnn-sw-map}
}
\end{figure}
A Bayesian Neural Network approach is now applied to perform the regression and create the surrogate model $\hat{u}_{DB}$ in the POD-NN framework, and the two test cases are the Ackley Function (2D), see Section \ref{sec:podensnn-bench-ackley}, and the Flood Predictions on the Mille Îles river, Section \ref{sec:podensnn-app-background}.  \par
The same datasets $\mathcal{D}=\{\bm{X}, \bm{v}\}$ are used on each case, and the setup remains the same. The prior is chosen to have the parameters $\pi_0=0.5$ and $\pi_2=0.1$ for both cases, while we picked $\pi_1=4.0$ for Ackley and $\pi_1=2.0$ for the flood modeling predictions. \par 
The trainable parameters $\bm{\theta}^{(j)}$ (weight or bias) of the $j$-th layer have been randomly initialized, with
\begin{equation}
\bm{\theta}^{(j)} = (\bm{\theta}^{(j)}_\mu, \bm{\theta}^{(j)}_\sigma) \sim \mathcal{N}\left(\bm{0}, \sqrt{\pi_0 \pi_1^2+(1-\pi)\pi_2^2}\bm{I}\right).
\end{equation}
The results of performing the regression using Bayesian Neural Networks are showcased in Figure \ref{fig:podbnn-ackley-graph-samples} and \ref{fig:podbnn-sw-map}, and are very similar to the one conducted in Section \ref{sec:podensnn-bench}, yet only requires one training time. \par 
The Ackley function case took 5 minutes and 24 seconds on a standard desktop CPU to reach a relative validation error of $RE_\textrm{val}=0.04\%$ after $N_e=70,000$ training epochs, and $RE_\textrm{tst}=0.03\%$ for the test error. One can see that the slices shown in Figure \ref{fig:podbnn-ackley-graph-samples} are very similar to the ones performed by the POD-EnsNN approach in Figure \ref{fig:podensnn-ackley-graph-samples}, with a similar proper fitting of the predicted mean, and a comparable uncertainty handling, hence validating the framework. \par
For the flood modeling case, the application of foremost interest, the training took 11 minutes and 36 seconds on a standard desktop CPU to reach a relative validation error of $RE_\textrm{val}=0.25\%$ after $N_e=200,000$ training epochs, and $RE_\textrm{tst}=0.26\%$ as well for the test error. These computing times are similar to the ensembles approach in a linear training setting. However, when parallelized as we did in Section \ref{sec:podensnn-app-background}, ensembles were faster by a factor of at least 5. \par
Figure \ref{fig:podbnn-sw-map} shows similar probabilistic flooding lines as Figure \ref{fig:podensnn-sw-map}, yet the Bayesian approach seems to produce larger confidence intervals, as it is depicted quantitatively by the measured distance on the second column between the CuteFlow solution and the upper bound of the confidence interval. \par
As for the POD-EnsNN, we inspected the uncertainties predicted out-of-distribution, and the results are displayed in Figure \ref{fig:podbnn-sw-in-n-out}. Nonetheless, one can note that the increase isn’t as drastic as for the Deep Ensembles, and our observations were that the prior parameters had a direct impact on this matter. \par
Documented source code will be made available at \href{https://github.com/pierremtb/POD-UQNN}{https://github.com/pierremtb/POD-UQNN}, on the \texttt{POD-BNN} branch.\par
% Since less precise results had been achieved when using a dual-output setting for the Bayesian NN, we resorted to manually set the \emph{aleatoric uncertainty} to a value $\sigma_{\textrm{init}}$, which would approximately correspond to the observed noise in the data in each case, and that we set as the standard deviation between the mean obtained by the Deep Ensembles in Section \ref{sec:podensnn-bench-ackley}-\ref{sec:podensnn-app-background} on the training points and the points themselves, resulting in $\sigma_\textrm{init}=2.76$ for the Ackley function, and $\sigma_\textrm{init}=0.24$ for the flood modeling application. One can note that any properly regularized model, including could be used to retrieve this estimation.\par
Additionally, quality training was harder to achieve for Bayesian Neural Networks compared to Deep Ensembles, since the convergence itself greatly depended in our experiments on numerical stability issues such as the coefficients to be inserted before or in the softplus function when ensuring positivity. The probabilistic layers and their uncertainty prediction was also dependent on the number of training epochs, with cases of uncertainties dropping when more epochs were performed. More practical details and handy insights in the implementation of BNN are discussed in \cite{keydana2019uncertaintytfp}, with examples in the R programming language.

\begin{figure}[t]
\vspace{-12pt}
  \centering
  \fbox{
  \hspace{0.15\textwidth}
   \includegraphics[width=0.42\textwidth]{images/podbnn_in_n_out.pdf}
  \hspace{0.15\textwidth}
  }
\\ \parbox{0.80\textwidth}{
    \caption{POD-BNN on the flooding case. Visualization of the average uncertainties for a range of inputs, with the two vertical black lines depicting the boundaries of the training and testing scope} \label{fig:podbnn-sw-in-n-out}
}
\end{figure}

==> content/poduqnn.tex <==
\emph{This chapter content is also available as a journal article, which is in the process of being submitted to the Journal of Computational Physics.}

\input{content/intro}

\input{content/reducingorder}
\input{content/learning}
\input{content/benchmarks-uq}
\input{content/applications}

\input{content/podbnn}
\input{content/podbnn-results}

\input{content/wrapup}

